Convolutional Networks in Visual Environments

The puzzle of computer vision might find new challenging solutions when we realize that most successful methods are working at image level, which is remarkably more difficult than processing directly visual streams. In this paper, we claim that their processing naturally leads to formulate the motion invariance principle, which enables the construction of a new theory of learning with convolutional networks. The theory addresses a number of intriguing questions that arise in natural vision, and offers a well-posed computational scheme for the discovery of convolutional filters over the retina. They are driven by differential equations derived from the principle of least cognitive action. Unlike traditional convolutional networks, which need massive supervision, the proposed theory offers a truly new scenario in which feature learning takes place by unsupervised processing of video signals. It is pointed out that an opportune blurring of the video, along the interleaving of segments of null signal, make it possible to conceive a novel learning mechanism that yields the minimum of the cognitive action. Basically, while the theory enables the implementation of novel computer vision systems, it is also provides an intriguing explanation of the solution that evolution has discovered for humans, where it looks like that the video blurring in newborns and the day-night rhythm seem to emerge in a general computational framework, regardless of biology.

==> Dissipation.tex <==

%Interestingly, we  prove that the gradual construction of the cognitive action on the basis %of a blurring of the video  turns out to be a method to track the optimal solution, thus %concluding that classic developmental issues in newborns turn out to be the outcome of %information-based laws more than biology.

%It might be the case that the baby reduced 
%visual acuity be the response of Nature to actually improve perceptual efficiency 
%by eliminating the ``information overload'' caused by too many extraneous 
%fine details, that are likely to overwhelm the infant?s cognitive system. 

% blurring as a way to determine the coefficients of the euler-lagrange eqs and enforce
% stability
Most of machine learning algorithms are developed in the framework of statistics,
so as the achievement of good generalization is strongly connected with the appropriate
selection of the samples to be used for learning. The approach to learning discussed
in this paper does not rely on a training set, but on the formalization of the life of the
agent in its own visual environment, so as there is no neat distinction between 
training and test sets. Clearly, we need to devise a different way of capturing the
consistency of the learning process that is not necessarily driven directly by statistical
principles that rely on sample complexity analyses. 
Interestingly, in the case of asymptotically stable Euler-Lagrange differential
equations and of finiteness assumptions on the visual information, 
the formulation given in this paper allows us to  establish links with statistical
consistency. This is due to the minimization property of the action that has
been derived in this paper. 

A natural way to express the finiteness  of visual information is to assume that the
video is an almost periodic~\cite{besicovitch1954almost} signal, that is for 
a certain small threshold  $\epsilon$ we can always find the spatiotemporal 
displacements $u(x,t) \in \R^{2}, \  v(x,t) \in \R^{+}$, and $\bar{t}$ such that
when $t > \bar{t}$ we have
\begin{equation}
	|C_{i}(x,t) - C_{i}(x-u(x,t),t-v(x,t))| < \epsilon.
\end{equation}
Notice that, for the spatial displacement we can also have $u(x,t)=0$, and it
must satisfy the consistency condition
$\forall x: \ \ 0 \leq |x-u(x,t)| \leq L$. For the temporal displacement
we assume that $v(x,t) < T$, which is essentially expressing the finiteness
of visual information. This condition can be given a correspondent form
in the case of the discrete retina discussed in Section~\ref{discretization-section}.
For any pair $(x,t)$ the input becomes $C_{ix}^{\sharp}(t)$
so as the previous almost periodicity condition becomes  
$|C_{ix}^{\sharp}(t) - C_{i,x-u(x,t)}^{\sharp}(t-v_{x}(t)))| < \epsilon$.
Now we show that this condition plays a crucial role in the consistency of
the learning process. From Eq.~(\ref{ForthOrderDiff}) we get
\begin{align*}
	q^{(4)}(t)+A(t)q^{(3)}(t)+B(t) q^{(2)}(t)+C(t) q^{(1)}(t)+D(t)q(t)+F(t,q(t))=0 \\
	q^{(4)}(t-v(t))+A(t-v(t))q^{(3)}(t-v(t)) +B(t-v(t)) q^{(2)}(t-v(t)) \\
	+C(t-v(t)) q^{(1)}(t-v(t)) +D(t-v(t))q(t) +F(t-v(t),q(t-v(t)))=0,
\end{align*}
If we define $q_{\delta}(t):=q(t)-q(t-v(t))$ then we get
\begin{align}
	q_{\delta}^{(4)}(t)+A(t)q_{\delta}^{(3)}(t)+B(t) q_{\delta}^{(2)}(t)
	+C(t) q_{\delta}^{(1)}(t)+D(t) q_{\delta}(t)=0.
\end{align}
If we use the $E_{t,\tau}$ operator of Eq.~(\ref{AveragingOperator}) and 
define $\bar{q_{\delta}}:=E_{t,\tau}(q_{\delta})$ then we get
\begin{align}
	\bar{q}_{\delta}^{(4)}(t)+A(t)\bar{q}_{\delta}^{(3)}(t)+B(t) \bar{q}_{\delta}^{(2)}(t)
	+C(t) \bar{q}_{\delta}^{(1)}(t)+D(t) \bar{q}_{\delta}(t)=0.
\end{align}
If this is asymptotically stable then as $t \rightarrow \infty$ we have
$ \bar{q}_{\delta}(t) \rightarrow 0$ which indicates that $\bar{q}(t)$
converges to a constant value. 

To sum up the dynamics corresponding to the introduction of blurring so as
to enforce causality results in the minimization of the action on any 
given interval. The almost periodicity assumption also ensures that the
minimum corresponds, for large intervals, to a solution that is 
independent of time. It turns out that the dependent on $t$ of the filter
parameters is in fact due to the learning process. The almost periodicity assumption
corresponds somewhat with a restriction on the information associated
with the visual stream. It is such a restriction that plays the crucial role
for an asymptotic time-invariant solution of $q(t)$. 





==> mydefs.tex <==

% For et al.'ing things
\newcommand{\etal}{{\em et al.\/}}
\def\annote#1{\par {\bf #1}\par}

\newcommand{\bbR}{{\mathbb{R}}}
\newcommand{\bbN}{{\mathbb{N}}}

%\def\NaturalSet{\mbox{I\hspace*{-0.16em}N}}
\def\RealSet{\mbox{I\hspace*{-0.16em}R}}

\def\NaturalSet{\mbox{$I\!\! N$}}
%\def\RealSet{\mbox{$I\!\!R$}}
%\def\func#1{\mbox{$#1(\cdot)$}}

\def\N{\mbox{$I\!\! N$}}
\def\R{\mbox{$I\!\!R$}}
\def\C{\mbox{\rm C}}

\def\QED{\protect{\flushright{$\Box$}}}
%\def\QED{\mbox{\rule[0pt]{1.5ex}{1.5ex}}}
%\def\qed{\hspace*{\fill}~\protect{\QED}}
%\def\ONE{\Huge{\bf 1}\hspace{-.1cm}\normalsize{\mbox {\bf I}}}
\def\ONE{{\bf 1}\hspace{-.1cm}{\mbox {\bf I}}}
\def\ZERO{\bf 0}

\def\sequence#1#2#3{#1^{#3\choose #2}}
\def\chain{\oplus}
\def\quantize#1{\ulcorner #1 \lrcorner}
\def\path{\leadsto}
\def\nil{\mbox{\boldmath $0$}} 
\def\ONE{\mbox{\boldmath $1$}} 
\def\BBox{\vrule height 1.2ex width 1.2ex depth -.1ex}
\def\warp{\bowtie}
\def\RealSet{\mbox{$I\!\!R$}}
\def\Kernel{\mbox{$I\!\!K$}}

\def\smap{F}
\def\gmap{\mbox{\Large{$\tau$}}}
\def\tmap{f}


\def\shape#1{\rm }
\def\ot{\overline{t}}
\def\osigma{\overline{\sigma}}
\def\Set{\mbox{$\mbox{\sc set}$}}
\def\Reset{\mbox{$\mbox{\sc reset}$}}
\def\Nil{\mbox{$\mbox{\sc nil}$}}
\def\Not{\mbox{$\mbox{\sc not}$}}
\def\False{\mbox{$\mbox{\sc false}$}}
\def\True{\mbox{$\mbox{\sc true}$}}

\def\Action{$\mbox{\boldmath ${\cal A}$}$}

\def\pa{\mbox{pa}}
\def\vert{\mbox{vert}}
\def\de{\mbox{de}}
\def\det{\mbox{det}}
\def\dim{\mbox{dim}}
\def\sign{\mbox{sign}}
\def\diag{\mbox{diag}}
\def\ln{\mbox{ln}}
%\def\arg{\mbox{\shape{n}\selectfont arg}}
\def\softmax{\mbox{softmax}}
\def\argmax{\mathop{\operator@font argmax}}
\def\argmin{\mathop{\operator@font argmin}}

\def\BA{\mbox{\boldmath $A$}}
\def\BB{\mbox{\boldmath $B$}}
\def\BC{\mbox{\boldmath $C$}}
\def\BD{\mbox{\boldmath $D$}}
\def\BG{\mbox{\boldmath $G$}}
\def\BF{\mbox{\boldmath $F$}}
\def\BI{\mbox{\boldmath $I$}} 
\def\BPhi{\mbox{\boldmath $\Phi$}}
\def\BR{\mbox{\boldmath $R$}}
\def\BS{\mbox{\boldmath $S$}} 
\def\BL{\mbox{\boldmath $L$}} 
\def\BTheta{\mbox{\boldmath $\Theta$}}
\def\BU{\mbox{\boldmath $U$}} 
\def\BH{\mbox{\boldmath $H$}} 
\def\BM{\mbox{\boldmath $M$}}
\def\BN{\mbox{\boldmath $N$}}
\def\BP{\mbox{\boldmath $P$}} 
\def\BT{\mbox{\boldmath $T$}}
\def\BV{\mbox{\boldmath $V$}} 
\def\BX{\mbox{\boldmath $X$}}
\def\BB{\mbox{\boldmath $B$}}
\def\BC{\mbox{\boldmath $C$}}
\def\BR{\mbox{\boldmath $R$}}
\def\BY{\mbox{\boldmath $Y$}} 
\def\BW{\mbox{\boldmath $W$}}
\def\BZ{\mbox{\boldmath $Z$}}
\def\B0{\mbox{\boldmath $0$}}
\def\Balpha{\mbox{\boldmath $\alpha$}}
\def\Ba{\mbox{\boldmath $a$}}
\def\Bbeta{\mbox{\boldmath $\beta$}}
\def\Bb{\mbox{\boldmath $b$}}
\def\Bc{\mbox{\boldmath $c$}}
\def\Bd{\mbox{\boldmath $b$}}
\def\Bgamma{\mbox{\boldmath $\gamma$}}
\def\Bdelta{\mbox{\boldmath $\delta$}}
\def\BDelta{\mbox{\boldmath $\Delta$}}
\def\Beta{\mbox{\boldmath $\eta$}}
\def\Be{\mbox{\boldmath $e$}}
\def\Bepsilon{\mbox{\boldmath $\epsilon$}}
\def\Bf{\mbox{\boldmath $f$}}
\def\Bn{\mbox{\boldmath $n$}}
\def\Blambda{\mbox{\boldmath $\lambda$}}
\def\Bg{\mbox{\boldmath $g$}}
\def\Bmu{\mbox{\boldmath $\mu$}} 
\def\Bnu{\mbox{\boldmath $\nu$}} 
\def\Bm{\mbox{\boldmath $m$}}
\def\Bo{\mbox{\boldmath $o$}}
\def\Bphi{\mbox{\boldmath $\phi$}}
\def\Bpi{\mbox{\boldmath $\pi$}}
\def\Bpsi{\mbox{\boldmath $\psi$}}
\def\Bpi{\mbox{\boldmath $\pi$}}
\def\Bp{\mbox{\boldmath $p$}}
\def\Bq{\mbox{\boldmath $q$}}
\def\Br{\mbox{\boldmath $r$}}
\def\Bs{\mbox{\boldmath $s$}}
\def\B\tau{\mbox{\boldmath $\tau$}}
\def\Btheta{\mbox{\boldmath $\theta$}}
\def\Bdelta{\mbox{\boldmath $\delta$}}
\def\Bomega{\mbox{\boldmath $\omega$}}
\def\Bu{\mbox{\boldmath $u$}}
\def\Bvarphi{\mbox{\boldmath $\varphi$}}
\def\Bvartheta{\mbox{\boldmath $\vartheta$}}
\def\Bvarsigma{\mbox{\boldmath $\varsigma$}}
\def\Bv{\mbox{\boldmath $v$}}
\def\Bw{\mbox{\boldmath $w$}} 
\def\Bxi{\mbox{\boldmath $\xi$}}
\def\Bx{\mbox{\boldmath $x$}}
\def\Bd{\mbox{\boldmath $d$}}
\def\By{\mbox{\boldmath $y$}} 
\def\Bzeta{\mbox{\boldmath $\zeta$}}
\def\Bz{\mbox{\boldmath $z$}}
\def\EQ{\!=\!}
\def\Given{\mbox{$\: \bigl | \bigr. \:$}}
\def\MAX{\mbox{\sc max}}
\def\MIN{\mbox{\sc min}}
\def\Overq{{\overline{q}}}
\def\Pr{\mbox{P}}
\def\given{\mbox{$\: | \:$}}

\def\vectw#1#2{\!\left[\!\!\begin{array}{r}#1\\#2\end{array}\!\!\right]\!}

\def\ivector#1{\sfmath{I}_{[#1]}}
\def\CalA{{\cal A}}
\def\CalB{{\cal B}}
\def\CalC{{\cal C}}
\def\CalD{{\cal D}}
\def\CalE{{\cal E}}
\def\CalF{{\cal F}}
\def\CalG{{\cal G}}
\def\CalH{{\cal H}}
\def\CalI{{\cal I}}
\def\CalJ{{\cal J}}
\def\CalL{{\cal L}}
\def\CalM{{\cal M}}
\def\CalN{{\cal N}}
\def\CalO{{\cal O}}
\def\CalP{{\cal P}}
\def\CalQ{{\cal Q}}
\def\CalR{{\cal R}}
\def\CalS{{\cal S}}
\def\CalT{{\cal T}}
\def\CalU{{\cal U}}
\def\CalV{{\cal V}}
\def\CalW{{\cal W}}
\def\CalX{{\cal X}}
\def\CalY{{\cal Y}}
\def\CalZ{{\cal Z}}
\def\VecCalE{{\cal{\vec{E}}}}
\def\Alphabet{{\cal A}}
\def\Real{\mbox{$\mathbb{R}$}}
\def\AND{\mbox{${\cal B}_\wedge$}}
\def\OR{\mbox{${\cal B}_\vee$}}

\def\istar{\mbox{$\CalI^\star$}}
% \def\EqDef{\doteq}
\def\EqDef{\buildrel \rm def \over =}

\def\RefFig#1{Figure~\ref{#1}}
\def\RefTab#1{Table~\ref{#1}}
\def\RefEq#1{(\ref{#1})}
\def\RefEqs#1#2{(\ref{#1},\ref{#2})}
\def\RefCh#1{Chapter \ref{#1}}
\def\RefSect#1{\S~\ref{#1}}
\def\RefSec#1{\S~\ref{#1}}
\def\RefSub#1{\S~\ref{#1}}
\def\RefDef#1{Definition~\ref{#1}}
\def\RefTh#1{Theorem~\ref{#1}}
\def\RefTh#1{Conjecture~\ref{#1}}
\def\cdw#1{{\em \underline{#1}}}


% An list-like environment that indents second, etc. lines of each item.
\newenvironment{defs}%
{\begin{list}{}{\setlength{\itemindent}{-\leftmargin}\setlength{\itemsep}{0pt}\setlength{\parsep}{0pt}}}%
{\end{list}}

% shrink and rotate everything for a two-pages on 1 printing using dvips.
%\input reduce.tex

% ``\heading'' is like a subsubsubsection, and takes a single argument.
% \newcommand{\heading}[1]{ \medskip
%         {\setlength{\parindent}{0in} \bf #1}
%         \nopagebreak
%         }

% ``\comment'' takes a single argument
\newcommand{\comment}[1]{}


% Local Variables: 
% mode: latex
% TeX-master: "main"
% End: 

